Spherical harmonics method for computing the image stress due to a spherical void

We develop an efficient numerical method for calculating the image stress field induced by spherical voids in materials. The method is applied to dislocation-void interactions in dislocation dynamics simulations. We obtain a complete set of basis functions for the solution of the image stress problem, as well as their corresponding displacement, stress, and traction fields in terms of the linear combination of spherical harmonics. Using the fast transformation between the real and spherical-harmonics spaces provided by the SHTOOLS package, the method is more efficient than other image stress solvers such as the finite-element method. This method can readily be extended for solving elasticity problems involving inclusions and inhomogeneities, contact between spheres, as well as other differential equations with spherical boundaries beyond elasticity.

==> util.tex <==
%% Useful items

\begin{comment}
\begin{itemize}
\item Bullet point one
\item Bullet point two
\end{itemize}

\begin{enumerate}
\item Numbered list item one
\item Numbered list item two
\end{enumerate}

\begin{table}[ht]
\centering
\begin{tabular}{l l l}
\hline
\textbf{Treatments} & \textbf{Response 1} & \textbf{Response 2}\\
\hline
Treatment 1 & 0.0003262 & 0.562 \\
Treatment 2 & 0.0015681 & 0.910 \\
Treatment 3 & 0.0009271 & 0.296 \\
\hline
\end{tabular}
\caption{Table caption}
\end{table}

\begin{figure}[ht]
\centering\includegraphics[width=0.4\linewidth]{placeholder}
\caption{Figure caption}
\end{figure}

\begin{equation}
\label{eq:emc}
e = mc^2
\end{equation}

\end{comment}

